Any-Width Networks

Despite remarkable improvements in speed and accuracy, convolutional neural networks (CNNs) still typically operate as monolithic entities at inference time. This poses a challenge for resource-constrained practical applications, where both computational budgets and performance needs can vary with the situation. To address these constraints, we propose the Any-Width Network (AWN), an adjustable-width CNN architecture and associated training routine that allow for fine-grained control over speed and accuracy during inference. Our key innovation is the use of lower-triangular weight matrices which explicitly address width-varying batch statistics while being naturally suited for multi-width operations. We also show that this design facilitates an efficient training routine based on random width sampling. We empirically demonstrate that our proposed AWNs compare favorably to existing methods while providing maximally granular control during inference.

==> figures/triangular-weights.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.4\linewidth}
        \includegraphics[width=\linewidth]{./images/vis/std-matrix.pdf}
        \caption*{\textbf{Traditional FC layer}}
    \end{subfigure}\quad
    ~
    \begin{subfigure}[b]{0.4\linewidth}
        \includegraphics[width=\linewidth]{./images/vis/tri-matrix.pdf}
        \caption*{\textbf{Triangular FC layer}}
    \end{subfigure}
    \caption{Comparing a TriFC layer to a traditional fully-connected layer.}
    \label{fig:trifc-vs-fc}
\end{figure}

==> sections/limitations.tex <==
\section{Limitations and Future work}
- Potentially harder training and more sensitivity to hyperparams, as seen in MobileNetV2 CIFAR10/100 experiments (did not happened with LeNet MNIST, FashionMNIST, Cifar10/100):

+ Accuracy: Low individual accuracies compare to S-Net baselines 

+ Param sensitivity: May require more tuning to achieve comparable accuracy, loss expoded for large LR (lr=0.1), more regularization needed (for example in the form of higher weight decay) etc.


% \begin{table*}[ht] 
% \begin{center}
%   \begin{tabular}{rccccc}
%     % \toprule
%   \hline
%     &&\multicolumn{4}{c}{Top-1 Validation Accuracy} \\
%     % \cmidrule(r){3-6}
%     Width        & FLOPS & Individual & Slimmable & Triangular (ours) & AWN (ours)\\ %(sandwich)
%     % \midrule
%   \hline
%   \hline
%     1.0$\times$  & 7.1M & 91.87 \% & 92.13 \% & 92.28 \% & 91.81 \%\\
%     0.75$\times$ & 4.1M & 91.58 \% & 91.73 \% & 92.03 \% & 91.91 \%\\
%     0.5$\times$  & 1.8M & 90.99 \% & 91.07 \% & 91.01 \% & 91.19 \%\\
%     0.25$\times$ & 0.5M & 89.68 \% & 89.45 \% & 89.11 \% & 89.08 \%\\
%     % \bottomrule
%   \hline
%   \end{tabular}
% \end{center}
% \caption{Classification results on FashionMNIST}
% \label{table:fashionMNIST-acc}
% \end{table*}

% \begin{table*}[ht] 
% \begin{center}
%   \begin{tabular}{rccccc}
%   \hline
%     % \toprule
%     &&\multicolumn{4}{c}{Top-1 Validation Accuracy} \\
%   \hline
%     % \cmidrule(r){3-6}
%     Width        & FLOPS & Individual & Slimmable & Triangular (ours) & AWN (ours)\\ %(sandwich)
%   \hline
%   \hline
%     % \midrule
%     1.0$\times$  & 10.6M & 82.46 \% & 80.75 \% & 81.1 \% & 80.02 \%\\
%     0.75$\times$ & 6.1M & 79.78 \% & 77.64 \% & 78.64 \% & 77.15 \%\\
%     0.5$\times$  & 2.8M & 75.83 \% & 73.01 \% & 73.88 \% & 71.96 \%\\
%     0.25$\times$ & 0.8M & 66.16 \% & 63.46 \% & 62.43 \% & 65.13 \%\\
%     % \bottomrule
%   \hline
%   \end{tabular}
% \end{center}
% \caption{Classification results on CIFAR-10}
% \label{table:cifar10-acc}
% \end{table*}

% \begin{table*}[ht] 
% \begin{center}
%   \begin{tabular}{rccccc}
%   \hline
%     % \toprule
%     &&\multicolumn{4}{c}{Top-1 Validation Accuracy} \\
%     % \cmidrule(r){3-6}
%   \hline
%     Width        & FLOPS & Individual & Slimmable & Triangular (ours) & AWN (ours)\\ %(sandwich)
%     % \midrule
%   \hline
%   \hline
%     1.0$\times$  & 10.6M & 53.62 \% & 51.19 \% & 53.44 \% & 53.14 \%\\
%     0.75$\times$ & 6.1M & 50.68 \% & 47.65 \% & 50.64 \% & 48.13 \%\\
%     0.5$\times$  & 2.8M & 44.83 \% & 42.28 \% & 43.85 \% & 40.51 \%\\
%     0.25$\times$ & 0.8M & 34.81 \% & 32.11 \% & 31.75 \% & 32.81 \%\\
%     % \bottomrule
%   \hline
%   \end{tabular}
% \end{center}
% \caption{Classification results on CIFAR-100}
% \label{table:cifar100-acc}
% \end{table*}


